How Far Can Disaggregation Go? A Design-Space Exploration of Attention-FFN Disaggregation for Efficient MoE LLM Serving

Modern large language model (LLM) inference has progressively disaggregated to keep pace with growing model sizes and tight TTFT and TPOT service-level objectives: from chunked-prefill aggregation, to prefill-decode (P/D) disaggregation, and most recently to operator-level Attention-FFN Disaggregation (AFD). This trend is especially important for mixture-of-experts (MoE) models, where memory-bound attention, compute-intensive expert FFNs, and MoE dispatch/combine communication create distinct resource demands. AFD further exposes this heterogeneity by placing attention and MoE-FFN execution on separate GPU groups. Each level of disaggregation deepens the scheduling design space across workload characteristics, resource allocation, and interconnect topology, raising the central question: when does each level actually pay off? We systematically characterize this trade-off for MoE inference across realistic workloads spanning input/output sequence lengths, prefix-KV reuse, and per-user latency constraints. Using chunked-prefill and P/D disaggregation as baselines, we study the benefits and limits of AFD at scale through a framework that fuses on-device kernel measurements with high-fidelity network simulation. Under strict TTFT/TPOT SLOs, AFD sustains around 4k tokens/s of system throughput on DeepSeek-V3.2 across chat, coding, and agentic-coding workloads, where non-AFD deployments are infeasible. We distill concrete takeaways for jointly optimizing throughput and interactivity, including how to partition attention and FFN across GPUs as a function of workload and model architecture, providing design principles for current rack- and cluster-scale deployments as well as future disaggregated AI infrastructure.

==> Sections/Background.tex <==
\section{Background and Motivation}

\subsection{Design-Space Exploration for Optimal Disaggregated Inference}
As model sizes continue to grow and new architectures emerge, the need for inference scheduling optimization has intensified, giving rise to an increasingly large design space. Finding the optimal scheduling strategy for large-scale disaggregated inference is critical to meet the stringent service-level latency and throughput requirements.

\textbf{The complex multi-dimensional search space:}
LLM inference scheduling spans multiple dimensions, encompassing diverse parallelism strategies as well as phase‑ and operator‑level disaggregation. Prior work explores parallelization across both data and model dimensions: data parallelism (DP) partitions input batches across devices, while sequence parallelism (SP) divides long‑context inputs; tensor parallelism (TP) and pipeline parallelism (PP) split model computation across devices, and Mixture‑of‑Experts (MoE) models further introduce expert parallelism (EP) to execute experts concurrently across nodes (\cref{fig:taxonomy}).
In large‑scale disaggregated deployments, multiple parallelism strategies across input, model, and expert dimensions can be composed to achieve optimal scheduling.
Beyond parallelism, recent systems such as Splitwise~\cite{splitwisesim2024} and DistServe~\cite{zhong2024distserve} advocate prefill–decode disaggregation, executing these phases on separate compute nodes to accommodate their heterogeneous execution characteristics. More recently, MegaScale‑Infer~\cite{zhu2025megascaleinfer} advances this direction by proposing fine‑grained operator‑level disaggregation within Transformer blocks, separating attention and FFN layers to better match their distinct compute and memory demands.

We further observe that workload characteristics significantly influence the choice of scheduling strategy. In particular, the input and output sequence lengths (ISL/OSL) and the effective context length can shift the optimal scheduling decision by a substantial margin, due to their impact on cross‑node data‑transfer volume and rates. For example, retrieval‑augmented generation (RAG) workloads—such as legal advisory chatbots—typically exhibit large context lengths and small ISLs. These workloads favor aggregated deployments, as frequent cross‑node data transfers in disaggregated systems incur high communication overheads. In contrast, workloads with long ISLs, common in code‑completion and code‑generation tasks, benefit more from asynchronous function decomposition (AFD), introducing an additional dimension into the scheduling design space.
\Cref{fig:dse} illustrates the Pareto‑optimal scheduling configurations for a \texttt{Qwen3‑30B‑A3B} model deployed on eight GPUs, with a fixed ISL of 4,000 tokens and an OSL of 500 tokens, while constraining time‑to‑first‑token (TTFT) to within \texttt{600ms}. The results demonstrate how the optimal scheduling choice varies with batch size, highlighting the combined influence of workload characteristics and system load in disaggregated inference environments. In this work, we systematically navigate this multi‑dimensional design space to identify latency‑optimal configurations for disaggregated inference deployments.

\textbf{The need for accurate modeling of disaggregated systems:}
Exploring a large design space by evaluating hundreds of candidate configurations is prohibitively expensive for large‑scale disaggregated inference systems, as demonstrated by prior work~\cite{xu2026aic, galvatron, alpa}. Consequently, accurate modeling of disaggregated architectures is essential to efficiently identify optimal scheduling strategies. NVIDIA’s AIConfigurator~\cite{xu2026aic} models compute and memory bandwidth characteristics across a wide range of modern GPUs and supports multiple parallelism strategies as well as coarse‑grained prefill–decode disaggregation. However, it lacks accurate estimation of cross‑node data‑transfer costs, which are critical for fine‑grained, operator‑level asynchronous function decomposition (AFD).
To address this limitation, we augment AIConfigurator with the AstraSim~\cite{astrasim} network simulator, resulting in AIConfigurator++ (AIC++), a disaggregated modeling framework that captures both compute and communication effects. AIC++ extends AIConfigurator into an event‑driven modeling framework that interacts with AstraSim to accurately estimate end‑to‑end latency by jointly modeling computation and cross‑node data movement in scale‑out, disaggregated inference platforms.
As shown in~\cref{xxx}, AIC++ exhibits significant divergence from AIConfigurator in estimating the performance of AFD configurations. By accurately accounting for data‑transfer latency, AIC++ identifies a superior scheduling configuration that reduces end‑to‑end latency by $x\%$ compared to AIConfigurator. These estimates are validated on a real system with eight H100 GPUs, underscoring the critical role of precise data‑transfer modeling in disaggregated inference scheduling.

\subsection{Operator placement in emerging heterogeneous architectures}
The emergence of architectures like nvidia Groq+GPU and intel Sambanova shifted the disaggregated paradigm by hosting heterogeneous compute nodes in the 
same scale-up interconnect as shown in~\cref{fig:taxonomy}.
Such heterogeneous clusters with high bandwidth scale-up interconnect can be efficiently leveraged for fine-grained AFD, where memory-bound attention operators can be computed in compute-nodes with larger memory capacity while compute-intensive FFN blocks benefit from accelerators with high arithmetic throughput.

\textbf{Compute-communication overlap to reduce compute idle times:}
The high frequency of data transfers inherent to AFD, particularly in the presence of high‑throughput compute nodes, necessitates efficient compute–communication overlap to minimize resource idle time. 
\textit{AIC++} explicitly incorporates interconnect topology and link duplex characteristics to micro‑batch AFD data transfers, thereby maximizing overlap across batches. In addition, it accounts for the heterogeneous throughput of individual compute nodes and structures the computation accordingly to maximize overall resource utilization.

\textbf{Precise placement of attention and ffn operators:}
Fine‑grained data transfers introduced by AFD can lead to significant interconnect congestion if attention and FFN operators are placed arbitrarily across a disaggregated infrastructure. Consequently, effective scheduling of fine‑grained operator disaggregation requires jointly reasoning about compute affinity and data‑movement costs—a challenge explicitly addressed in our work. In particular, optimal operator placement must account for compute–communication overlap by co‑locating operators with high data‑exchange intensity on nearby or tightly coupled compute nodes. Going beyond prior approaches that primarily model heterogeneous architectures, our work jointly optimizes operator placement by explicitly considering interconnect congestion, identifying optimal mappings of attention and FFN operators that maximize overall system efficiency.










\begin{figure}[t]
    \centering
    \includegraphics[width=8.5cm]{ASPLOS2027_Main/Include/Figures/assignment_8gpus.pdf}
    \vspace{-8pt}
    \caption{assignment of 8GPUs}
    \label{fig:8gpus_assignment}
\end{figure}

\begin{figure}[t]
    \centering    \includegraphics[width=8.5cm]{ASPLOS2027_Main/Include/Figures/search_space_disagg_serve.pdf}
    \vspace{-8pt}
    \caption{search space}
    \label{fig:search_space_disagg_serve}
\end{figure}


\subsection{LLM Serving Characteristics At-Scale}
As model sizes continue to grow and new architectures emerge, the need for inference optimization has intensified, giving rise to an increasingly large and complex design space. The key dimensions of the design‑space exploration (DSE) objectives are as follows:

\subsubsection{Parallelism of LLM models}
\begin{itemize}
    \item Discuss TP,PP,EP,SP etc. in a broad distributed deployment.
\end{itemize}
As modern LLMs exceed the compute and memory limits of a single accelerator, distributed execution across multiple devices has become essential. Prior work proposes several complementary parallelization strategies: data parallelism (DP), pipeline parallelism (PP), tensor parallelism (TP), expert parallelism (EP) for MoE models, and sequence parallelism (SP). Each operates along a different axis—data, layers, tensors, experts, or tokens—and exhibits distinct compute–memory trade‑offs depending on model size, hardware topology, and sequence length. Importantly, these strategies are not mutually exclusive and can be composed to form compound parallelization schemes, giving rise to a large and complex design space for large‑scale deployments.

\TODO{do we need to create a mathematical value in terms of k gpus?}

\subsubsection{Token-level batching of inference requests}
\begin{itemize}
    \item Better SLO with reduced starvation of multiple requests.
    \item Long contexts require token-level splitting for faster prefill phase.
    \item Opportunity to interleave the decode phase for multiple requests.
\end{itemize}
Modern LLM serving workloads exhibit substantial heterogeneity across requests, including variations in arrival patterns, prompt lengths, and response lengths.
Continuous batching enables requests to dynamically join and leave execution batches at token boundaries, rather than requiring batches to be fixed at dispatch time, thereby improving utilization under dynamic arrivals. Chunked prefill, in contrast, partitions long prompts into fixed‑size chunks to mitigate extended prefill latency, allowing decode operations for latency‑critical requests to execute concurrently with prefill. Together, these scheduling techniques interleave execution across requests and significantly improve SLOs, particularly for long‑context workloads.


\subsubsection{Phase-level disaggregation}
\begin{itemize}
    \item Prefill and decode phase have different compute and memory characteristics.
    \item Prefill phase is compute-intensive while the decode phase require hardware with large memory bandwidth and capacity for storing large KV cache which scales with batch size and long contexts.
    \item Efficient execution requires compute-intensive hardware for prefill and memory-intensive hardware for decoder block.
\end{itemize}
The prefill and decode phases of LLM inference exhibit fundamentally different execution characteristics. Prior systems such as Splitwise and DistServe identify this heterogeneity and propose disaggregating the two phases across separate platforms. The prefill phase is compute‑intensive, favoring accelerators with high compute throughput, whereas the decode phase is predominantly memory‑bound and benefits from high memory bandwidth. Prefill–decode disaggregation further requires a high‑bandwidth, low‑latency interconnect to efficiently transfer large KV caches between phases. Overall, this approach improves resource utilization, reduces head‑of‑line blocking, and enables better latency SLOs under long‑context and multi‑tenant workloads.

Taxonomy of different Disaggregated Inference and the real-system evaluated performance.

\subsubsection{Operator-level disaggregation}
\begin{itemize}
    \item Even within the transformer block, the attention and ffn blocks have different compute-memory characteristics.
    \item This is more pronounced in MoE models - with a large number of experts (FFN blocks).
    \item Attn-ffn split to heterogeneous hardware can lead to an optimal execution characteristics.
    \item However, this split requires data-transfer across devices at a finer granularity.
    \item Choosing the specific attn and ffn layers is critical in large scale-out designs. 
    \item This work proposes optimal scheduling of individual attn and ffn layers to minimize overall latency and provides a strategy to scale it up and out for large models in a heterogeneous hardware (like LPU + Grok designs).
\end{itemize}
The attention (ATTN) and feed‑forward network (FFN) components of transformer models exhibit distinctly different compute–memory characteristics. Attention is predominantly memory‑bound, whereas FFN layers are compute‑intensive; disaggregating these operators can therefore reduce GPU under‑utilization, particularly in large‑scale and MoE‑based architectures.
However, operator‑level disaggregation introduces substantial data‑movement overhead, as intermediate activations must be transferred across the interconnect.
In this paper, we characterize attention–FFN disaggregation (AFD) across a range of LLM architectures and demonstrate how judicious operator placement in large compute clusters improves system efficiency. Furthermore, we leverage heterogeneous hardware platforms by mapping compute‑intensive and memory‑intensive operators to specialized devices, achieving improved end‑to‑end latency and overall resource efficiency.

\subsection{Framing and solving a complex DSE problem}
\begin{itemize}
    \item LLM efficiency plays a key role to reduce compute and energy requirement for each token generation.
    \item LLM inference is spread across all these different dimensions.
    \item choosing an operating point is a large DSE problem and depends on the model size, architecture, input context length and a variety of factors.
    \item Explain the pareto optimal plot (Figure 6) for homogeneous hardware.
    \item How this work enables efficient LLM serving across all these dimensions by deriving the pareto-frontier.
    \item Motivate that the DSE becomes more complex in the presence of heterogeneous hardware.
    \item How to make the DSE a future proof by solving a fundamental operator level AFD disaggregation. 
\end{itemize}

\subsection{Challenges and opportunities.}
\begin{itemize}
    \item Challenge 1: Accurate modeling of large-scale systems - Needed for precise computation, communication and memory costs.
    \begin{enumerate}
        \item Leverage AIConfigurator for baseline designs - augment it into an event-driven simulator. 
        \item Extend Astrasim to accurately estimate the commmunication cost for fine-grained disaggregation. 
        \item Modeling heterogeneous hardware combinations with independent bandwidth of scale-up and scale-out interconnects - enables precise positioning of each attention and ffn blocks.
    \end{enumerate}
    \item Challenge 2: Creating a DSE for future workloads and designs:
    \begin{enumerate}
        \item Operator-level split enables updating workloads (having transformer layers) to the number of blocks. 
        \item The DSE enables identify clear bottlenecks of key sub-blocks enabling accurate design of future hardware.
        \item Several existing and experimental network topologies are already integrated in Astrasim. Design can easily scale-up or scale-out with this interconnect simulator. 
    \end{enumerate}
\end{itemize}

Motivation of the next-generation serving and bottleneck using afd. For MoE servin
\TODO{running this on vllm and Dynamo, some of them are already captured through aiconfigurator} 


==> Sections/Design_old.tex <==
\subsection{AIConfigurator}
AIConfigurator is good at configuration search under a fixed serving point, but it does not model the AFD-specific communication path or network-sensitive overlap behavior. We therefore extend AIConfigurator with an AFD-aware execution model and a calibrated network backend derived from Astra-sim, enabling it to reason about when AFD is beneficial and when communication overturns its gains.

\subsection{AFD Design}

AIConfigurator ships with a curated pool of measurements collected from a
wide range of production-class clusters, spanning NVIDIA A100, H100, H200,
and the latest B200 platforms. The dataset is organized at the operator and
kernel level, covering the workhorse primitives of modern LLM serving—dense
GeMMs, FlashAttention variants, fused MoE kernels, and NCCL collectives
(all-reduce, all-to-all, dispatch/combine). For configurations that fall
outside the measured grid (e.g., uncommon shapes, untested parallelism
degrees, or mixed-precision variants), AIConfigurator falls back to one of
two extrapolation strategies: (i) an \emph{analytical performance model}
augmented with empirically calibrated correction factors that absorb
hardware- and kernel-specific inefficiencies, and (ii) a
\emph{learning-based regression model} trained on the measured corpus that
predicts unobserved points while preserving the non-linear scaling trends
observed in the underlying hardware. Both pathways have been validated to
align with on-device measurements at high fidelity, allowing AIConfigurator
to serve as a trustworthy oracle for compute-side cost estimates across the
full design space we sweep in this work.

AIConfigurator on its own is well-suited to configuration search at a
\emph{fixed} serving point, but it does not natively model the AFD-specific
communication path nor the network-sensitive overlap behavior that arises
when attention and expert FFN computations live on physically disjoint GPU
groups. We therefore extend AIConfigurator with an AFD-aware execution
model and pair it with a calibrated network backend derived from
ASTRA-Sim, which faithfully captures topology, link bandwidth, and
collective scheduling on multi-tier scale-up/scale-out fabrics. 

\begin{itemize}
    \item Separate out the attention and ffn onto separate GPUs and has the memory tracker of the independent stages
    \item 
    
\end{itemize}

\subsubsection{Batch Overlap (BO) in AFD}

\paragraph{Pipeline structure.}
As shown on the right of \autoref{fig:Batch_overlap}, AFD execution decomposes
into four stages mapped onto independent compute and communication resources.
Following the MoE workflow on the left of the same figure, Stage~1 performs
the attention computation on the attention NPUs. Stage~2 \emph{pre-dispatches}
the post-attention hidden states, together with their top-$k$ routing
metadata, from the attention side to the matching experts via the intra- or
inter-node network links. Stage~3 executes the MoE/FFN kernels on the FFN
NPUs—primarily the gate/up/down GEMMs and the activation function. Stage~4
combines the partial expert outputs and ships them back to the attention side
through the reverse network path.

Because attention and expert MoE/FFN computations live on disjoint NPUs,
attention-to-expert traffic uses the egress link on the attention side and
the ingress link on the FFN side; the expert-to-attention reply uses the
opposite pair. On modern accelerator fabrics that expose
full-duplex links (e.g., InfiniBand and NVLink), the two communication
directions proceed concurrently and a \emph{4-stage} pipeline is realizable.
When only half-duplex links are available, the two directions contend for
the same wire and we collapse Stages~2 and~4 onto a single shared communication
stage, yielding a \emph{3-stage} pipeline.

\paragraph{Modeling in AIConfigurator++.}
To capture this behavior inside the AIConfigurator backend simulator, we
divide the per-step token budget ($\text{batch\_size} \cdot \text{isl}$) into
$M$ microbatches, where $M$ matches the pipeline depth ($M{=}3$ for the
half-duplex schedule and $M{=}4$ for the full-duplex schedule). For each
microbatch, we query AIConfigurator's GPU-cluster--measured cost database for
both the attention and the MoE/FFN kernels at the per-microbatch shape
($\text{batch\_size} \cdot \text{isl} / M$), which preserves the non-linear
scaling cost of small GEMMs and the collectives.

Let $s_i$ denote the measured per-microbatch cost of stage $i$ aggregated
across all $L$ transformer layers, and let $s_{\max}=\max_i s_i$ be the
bottleneck stage. Under steady-state cross-layer pipelining, the bottleneck
stage processes all $M$ microbatches back-to-back, while every non-bottleneck
stage contributes only a one-time pipeline-fill bubble of $s_i/L$ (charged
once for the whole run, not once per layer, matching the cross-layer
schedules adopted by MegaScale-Infer and Step-Fun). The end-to-end pipelined
latency is therefore
\begin{equation}
\label{eq:bo-pipe}
t_{\text{pipe}} \;=\; M \cdot s_{\max} \;+\; \sum_{i \,:\, s_i \neq s_{\max}} \frac{s_i}{L}.
\end{equation}
The first term captures the saturated steady state on the bottleneck
resource; the second term accounts for the fill/drain bubble across the
non-bottleneck stages in the pipeline execution. We
implement Eq.~\eqref{eq:bo-pipe} for both prefill and decode in
allowing
AIConfigurator++ to reason the cost of computation and communication under the batch overlap. 

==> Sections/Introduction.tex <==
\section{Introduction}

% Introduction flow:
% 1. Rise of agentic workloads with long context, multi-turn generation, MoE models etc. Explain efforts for scheduling long contexts - Continuous batching, Chunked Prefill.
% 2. The above techniques work on a single device. Introduce disaggregated serving - Specifically talk about prefill- decode disaggregation.
% 3. However, MoE workloads have sparse attention matrices - leading to GPU underutilization in the decode phase. Hence, there is a requirement of attention-ffn split - as proposed by Megascale- infer. - Even larger scale, Best scenario for Afd.
% For AIConfigurator 
% 3 (Key takeaway) - We have this three dimensions - token, operator, stage.
% 4 [Characterization] Different workloads and hardware wishlist. Showcase the need of Astrasim integration and the choice of AIconfigurator. ENLIST KEY CHALLANGES! 
% 4 [Sw effort] Start by workload for a given device - Characterization effort on what works best when.
% 5 [Hw effort] Tuning the hardware configuration for different workload types. Try out heterogeneous hardware combinations and (maybe) future hardware simulation with tuning AIConfigurator. Best HW - Rubin CPX for future work. 
% 6 Case study - 8 GPUs [ 4P + 4D] - If you place AFD in an unoptimal - Same scaleup domain - 2 Prefill (scale up ) + 2 Decode (scale out) vs. 1P+D (scale up) + 1P+D (Scale down). Multi-tier network transfer. AF>>PD for GPU. 
% Fine-grained placement of operators - 
% 6 List contributions - How this effort works to solve the mentioned challenges. 



% Questions:
% - Are we performing a DSE study on the three segregation dimensions?
% - Difference between Megascale-infer and this work?
% - Justify the usage of simulator.

% Introduction of emerging applications and architecture blocks that mandate disaggregated serving
The rise of large-scale agentic workloads—often involving hundreds of billions of parameters and multi‑turn generation over long contexts—has exposed a critical infrastructure bottleneck. Specifically, the heterogeneous compute and memory‑bandwidth demands across different components of agentic large language models (LLMs) lead to persistent resource imbalance, resulting in either idle compute units or under‑provisioned memory bandwidth.

Early approaches, such as chunked prefill (e.g., Sarathi~\cite{agrawal2023sarathi}) and continuous batching, recognize the fundamental imbalance between the compute‑intensive prefill phase and the memory‑bound decode phase in LLM inference, and mitigate it by partitioning execution into smaller units to enable more efficient scheduling on a single device.

As context lengths grow in multi‑turn agentic workloads, co‑locating both prefill and decode stages on a single device becomes increasingly infeasible. Long prefill executions monopolize compute resources, bottlenecking the decode stage, inflating inference cost, and preventing the system from meeting latency SLOs.
Phase-level disaggregation systems, such as Splitwise~\cite{patel2023splitwise} and DistServe~\cite{zhong2024distserve}, physically separated the Prefill and Decode stages to reduce resource interference.

While prefill–decode disaggregation alleviates SLO violations caused by long prefill executions by separating the decode stage, the underlying compute–memory imbalance persists in emerging large‑scale models - especially in Mixture-of-Experts (MoE) architectures as observed by MegaScale‑Infer~\cite{zhu2025megascaleinfer}.
The fundamental bottleneck stems from the intrinsic computational heterogeneity within the Transformer blocks - a key component in these large-language models (LLMs). 
Attention across variants such as Multi-Head Attention (MHA) \cite{ashish2017attention}, Grouped-Query Attention (GQA) \cite{hudson2019gqa}, and Multi-Latent Attention (MLA) \cite{deepseekai2024deepseekv2} is fundamentally memory-bound and heavily dependent on KV-cache capacity and movement. In contrast, the Feed-Forward Network (FFN), dominated by GEMM operations and activation processing, is primarily constrained by raw compute throughput ($FLOPS$).
By decoupling memory bandwidth-intensive attention operators from compute-intensive FFN operators, AFD enables independent scaling and hardware specialization for the two dominant and heterogeneous component of Transformer execution. 
~\Cref{fig:taxonomy} illustrates the spectrum of segregation granularities in LLM inference. Continuous batching and chunked prefill partition tokens across multiple inference steps while operating on a single device; prefill/decode (P/D) disaggregation separates these stages across heterogeneous hardware; and attention/FFN disaggregation (AFD) performs operator‑level segregation within transformer layers. However, the optimal segregation along the token, phase and operator dimension is dependent on the underlying architecture, model size, parallelism strategies and workload characteristics along with the underlying hardware configuration creating a large design space spanning across software and hardware.

\textbf{Multiple Disaggregation Axes Yield a Large Design Space:}
This paper investigates this design-space exploration (DSE) to compose an optimal scheduling for a wide variety of popular model architectures including large-scale MoE models. 
Specifically, this paper analyzes how Attention-FFN Disaggregation (AFD) as proposed by recent works like MegaScale-Infer~\cite{zhu2025megascaleinfer} can be used to efficiently scale workloads to existing heterogeneous compute backends like Rubin CPX and even future hardware. 
To enable a comprehensive exploration of the design space, we employ \toolns, an enhanced co-design framework built on NVIDIA AIConfigurator~\cite{xu2026aic}, which integrates kernel-level metrics with the AstraSim network simulator for accurate interconnect modeling. 
Grounded in a customized vLLM \cite{kwon2023vllm} prototype that implements AFD execution, \tool combines kernel-level performance measurements with simulation to model future architectures. Using this enhanced framework, we examine the co-design implications of operator-level separation across both homogeneous GPU clusters optimized for inter-operator communication and heterogeneous systems that incorporate specialized Attention accelerators.
With this new framework, this paper identifies substantial heterogeneity across the internal operators of the Transformer and exploits this structure to enable fine-grained disaggregation, achieving significantly greater compute–memory overlap than existing approaches.

\textbf{Finding the optimal AFD disaggregation requires careful system modeling:}
In addition to faithfully modeling the Attention-FFN disaggregation with \toolns, we characterize different Transformer architectures - 
including dense layers, sparse attention (ex., Deepseek) etc.,
sweep across workloads with different context lengths - ranging from chatbots, to multi-turn code generation. 
Our characterization provides valuable insights into scenarios where AFD is most applicable and configurations which maximize the compute-communication overlap for maximum efficiency. 
It also provides additional insights on the applicability of heterogeneous hardware components on various workloads, model size and architecture.

\textbf{Heterogeneous hardware can optimize AFD disaggregation:}
Finally, we showcase how heterogeneous hardware configuration can improve efficiency of different operators. For instance, the attention phase requires higher memory bandwidth and memory higher capacity to support a large KV cache for long contexts - a task 
that is fit for recent nvidia GPUs. 
On the other hand, the compute-intensive FFN blocks can be scheduled to high-density GEMM blocks with a large SRAM - similar to the recently announced LPU-Groq architecture. 
However, we additionally answer questions on the efficiency of wide EP architectures in NVL-72 systems or if we need large HBMs for Rubin CPX designs. 
This paper takes a systematic approach and focus on the design choices of future architecture based on the operators.

\textbf{Optimal operator placement is key to maximize disaggregation benefits:}

In summary, this paper makes the following contributions:
\begin{itemize}
    \item We create a design framework that extends the AIConfigurator execution models to include Astrasim network model to study the impact of Attention-FFN disaggregation (AFD).
    \item We perform a DSE to find the optimal scheduling across token, phase and operator-level disaggregation. [ Talk about operator placement] [Cross node order]
    [AFD ; PD; TP/EP]
    \item We perform two case-studies showcasing the impact of context length scaling and future architectural design. 
\end{itemize}

\begin{comment}
    

% Old Introduction 
To study the design space, we build AIConfigurator++, an enhanced co-design framework built on NVidia AIConfigurator~\cite{xu2026aic} and the Astra-sim network simulator.
Grounded in a customized vLLM \cite{kwon2023vllm} prototype that implements AFD execution, AIConfigurator++ combines kernel-level performance measurements with simulation to model future architectures. Using this enhanced framework, we examine the co-design implications of operator-level separation across both homogeneous GPU clusters optimized for inter-operator communication and heterogeneous systems that incorporate specialized Attention accelerators.


While prior work treats the transformer as a monolithic execution unit, this paper identifies substantial heterogeneity across its internal operators and exploits this structure to enable fine‑grained disaggregation, achieving significantly greater compute–memory overlap than existing approaches.





Scaling large language models (LLMs) to hundreds of billions of parameters has exposed a critical infrastructure bottleneck. The rise of agentic workloads, which require substantial token generation for iterative reasoning, places increasingly stringent demands on inference that traditional aggregated serving can no longer satisfy efficiently. A key source of this inefficiency is the intrinsic computational heterogeneity within Transformer blocks. Attention across variants such as Multi-Head Attention (MHA) \cite{ashish2017attention}, Grouped-Query Attention (GQA) \cite{hudson2019gqa}, and Multi-Latent Attention (MLA) \cite{deepseekai2024deepseekv2} is fundamentally memory-bound and heavily dependent on KV-cache capacity and movement. In contrast, the Feed-Forward Network (FFN), dominated by GEMM operations and activation processing, is primarily constrained by raw compute throughput ($FLOPS$).

System optimizations have progressively evolved to address these bottlenecks. Early techniques such as continuous batching and chunked prefill (e.g., Sarathi \cite{agrawal2023sarathi}) focused on maximizing single-device efficiency. Later, phase-level disaggregation systems, such as Splitwise \cite{patel2023splitwise} and DistServe \cite{zhong2024distserve}, physically separated the Prefill and Decode stages to reduce resource interference. However, these approaches still treat each Transformer layer as a monolithic unit and therefore do not address the substantial heterogeneity between its internal operators.

This paper investigates Attention-FFN Disaggregation (AFD) as the next logical step in the evolution of LLM serving. By decoupling memory-bound Attention operators from compute-intensive FFN operators, as proposed in frameworks such as MegaScale-Infer \cite{zhu2025megascaleinfer}, AFD enables independent scaling and hardware specialization for the two dominant components of Transformer execution. To study this design space, we use \textcolor{red}{ AIConfigurator++ ??}, an enhanced co-design framework built on NVIDIA AIConfigurator \cite{xu2026aic} and the ASTRA-sim \cite{astrasim} network simulator. Grounded in a customized vLLM \cite{kwon2023vllm} prototype that implements AFD execution, AIConfigurator++ combines kernel-level performance measurements with simulation to model future architectures. Using this enhanced framework, we examine the co-design implications of operator-level separation across both homogeneous GPU clusters optimized for inter-operator communication and heterogeneous systems that incorporate specialized Attention accelerators.


%% Challenge - lots of open questions. 
Figure1(a) demonstrates the taxonomy for different disaggregation stages.  



Understanding and addressing such questions is essential for advancing the scalability, efficiency, and reliability of current and next-generation LLM serving platforms as they become foundational to a broad range of industrial, scientific and societal applications ranging from interactive assistants to enterprise automation.

%This creates a complex design space where trade-offs arise between batching and responsiveness, memory footprint and model fidelity, parallelism and scheduling efficiency, as well as energy consumption and service-level objectives. Building effective inference platforms is therefore not merely a systems engineering challenge—it is fundamental to unlocking the economic and societal value of LLMs in domains ranging from 


%% No clear way of navigating the design space and design points. A line about past works
Unfortunately, there is a lack of systematic methodology to navigate the end-to-end co-design space of multi-stage LLM inference platforms today. There have been several recent efforts focusing on modeling the design-space of core model execution for LLM inference (i.e., prefill and decode). These studies have explored hardware level requirements~\cite{cho2024llmservingsimhwswcosimulationinfrastructure,bambhaniya2024demystifying, zhang2023hardware}, new system architectures such as disaggregated GPU pools~\cite{patel2023splitwise,zhong2024distserve} and memory pools~\cite{cho2024llmservingsimhwswcosimulationinfrastructure}, and impact of scheduling and batching optimizations~\cite{agrawal2024vidurlargescalesimulationframework}.
%There also exist simulators for modeling detailed communication behavior for scale-up/scale-out fabrics (such as collective algorithms and congestion control)~\cite{astrasim,astrasim_doc_ns3}. 

\end{comment}

==> Sections/Introduction_new.tex <==
\section{Introduction}

% Narrative hook on agentic LLMs being a heterogeneous scalability problem
The rapid scaling of agentic large language models (LLMs) has enabled the adoption of AI for decision‑making across a wide range of domains, including code generation, multi‑turn reasoning over complex problems, and autonomous task execution.
However, the scale of modern agentic models— characterized by hundreds of billions of parameters and long input contexts—leads to substantial KV‑cache footprints, necessitating deployment across multiple compute nodes with large memory capacity.
Moreover, as model architectures and workloads become increasingly heterogeneous, existing serving paradigms struggle to balance performance, efficiency and scalability.

% Focus on what is the key problem of agentic LLMs 
A key challenge arises from the heterogeneous execution characteristics of model architecture components, which place conflicting demands on compute, memory, and communication resources.
Prior systems have attempted to mitigate these effects through batching~\cite{agrawal2023sarathi, yu2022orca}, pipelining or coarse-grained 
prefill-decode phase disaggregation~\cite{zhong2024distserve,patel2023splitwise}.
However, such approaches implicitly treat key model components like transformers as a monolithic unit, obscuring fine-grained trade-offs that emerge at scale.

% Narrow the scope further into the exact problem tackled by this paper.
The fundamental bottleneck arises from intrinsic computational heterogeneity within Transformer blocks as observed by MegaScale-Infer~\cite{zhu2025megascaleinfer} - particularly for mixture-of-experts (MoE) model architectures.
Attention mechanisms—including Multi‑Head Attention (MHA)~\cite{ashish2017attention}, Grouped‑Query Attention (GQA)~\cite{hudson2019gqa}, and Multi‑Latent Attention (MLA)~\cite{deepseekai2024deepseekv2}—are fundamentally memory‑bound, dominated by KV‑cache capacity and data movement, whereas the Feed‑Forward Network (FFN) is primarily compute‑bound, constrained by GEMM throughput and activation processing.
Fine‑grained disaggregation of \textit{Attention} and \textit{FFN} layers across heterogeneous hardware with distinct compute–memory characteristics enables independent scaling and specialization of these dominant Transformer components, resulting in efficient, scalable, and high‑performance LLM inference.

% The GAP statement - what is not studied and the key challenge tackled by this work
Despite the growing importance of large‑scale model serving, the interaction between fine-grained operator‑level heterogeneity, scheduling decisions, and system‑level performance remains poorly characterized. 
In particular, it is unclear how fine‑grained disaggregation strategies should be designed and deployed across heterogeneous large-scale hardware infrastructures.
Addressing this gap is essential for enabling scalable and efficient AI systems in future computing environments.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]
    {ASPLOS2027_Main/Include/Figures/Contribution_overview.drawio.pdf}
    \vspace{-1em}
    \caption{Optimal operator placement in a heterogeneous scale-out compute architecture\AB{Lets have legends in the figure regarding Pa Pf, Da, Df}}
    \vspace{-2em}
    \label{fig:taxonomy}
\end{figure}

% Conceptual contributions: 
% 1. Formulation of the DSE problem
This paper presents a systematic study of \textit{Attention-FFN} disaggregation (AFD) in large-scale AI serving systems. 
We begin by examining inference parallelism across three dimensions: token‑level parallelism (e.g., tensor, data, pipeline, sequence, and expert), phase‑level prefill–decode disaggregation, and operator‑level attention–FFN disaggregation. 
We formulate the selection of an optimal inference execution point as a design‑space exploration (DSE) problem that models operator‑level computational heterogeneity and inter‑node data‑movement costs across distributed architectures to identify the most efficient and high‑performance LLM inference configuration.

% 2. Building the AIConfigurator++ framework
Next, we develop \tool (\textit{\toolabbr}), an enhanced co-design framework for evaluating design points within this DSE. While NVIDIA AIConfigurator (\textit{\toololdabbr})~\cite{xu2026aic} provides a basis for system exploration, it does not model distributed network behavior in detail. \toolabbr extends \toololdabbr  with support for AFD analysis and integrates ASTRA-Sim~\cite{astrasim}, an event-driven distributed network simulator, to capture data-movement costs across distributed architectures.
Grounded in a customized vLLM \cite{kwon2023vllm} prototype that implements AFD execution, \toolabbr combines kernel-level performance measurements with simulation to model future architectures. 
Using this enhanced framework, we examine the co-design implications of operator-level separation across both homogeneous GPU clusters optimized for inter-operator communication and heterogeneous systems (Groq + LPU) that incorporate specialized compute-intensive FFN accelerators.

% 3. Modeling and impact of AFD
Finally, we observe that the placement of \textit{Attention} and \textit{FFN} operators plays a decisive role in determining overall system efficiency, driven primarily by data‑transfer and communication overheads—particularly in large scale‑out deployments. We further introduce optimal micro‑batching stages that maximize compute–communication overlap, thereby reducing GPU under‑utilization. Through detailed modeling with \toololdabbr, we precisely identify these execution bottlenecks and characterize the impact of operator‑level Attention–FFN disaggregation (AFD), as well as its interaction with token‑level and phase‑level disaggregation strategies.

% A sneek-peek into the evaluation, analysis and insights
Our evaluation uncovers several key insights into optimal LLM serving configurations, many of which are highly sensitive to model architecture, workload characteristics, and the underlying system infrastructure. First, we observe that operator‑level Attention–FFN disaggregation (AFD) is beneficial primarily for large Mixture‑of‑Experts (MoE) models with sparse‑attention layers, where the compute intensity of the FFN outweighs the associated communication costs. Using the TODO‑MoE model on an 8‑GPU system, AFD improves throughput by $x\%$ compared to non‑AFD deployments. Second, we find that operator placement is critical in further amortizing communication overheads: an optimally placed AFD configuration achieves an additional $xx\%$ throughput gain over a naive placement strategy. These benefits amplify in large scale‑out settings, as demonstrated through simulations using AstraSim. Finally, the pronounced compute–memory heterogeneity at the operator level highlights the necessity of heterogeneous compute platforms in future inference architectures. Through a targeted architecture search case study, we show that heterogeneous designs—such as Groq+LPU—are optimal for large‑scale MoE models with sparse‑attention layers. We further report optimal system configurations across a range of LLM architectures.

% Summerize the broad impact of this work
Beyond AI serving, our findings point to a broader design principle for distributed computing systems: as workloads grow increasingly heterogeneous, performance optimization must evolve from coarse‑grained abstractions toward fine‑grained, operator‑level disaggregation. This shift necessitates future architectures built from heterogeneous hardware components, each tightly aligned with the compute–memory characteristics of specific operators. Looking ahead, we envision disaggregated, modeling‑driven frameworks such as \tool playing a central role in enabling next‑generation computing platforms to precisely select optimal inference serving strategies across a wide spectrum of current and emerging AI architectures.

\AB{We need to have a result teaser early on this page.}
\SB{I agree. Especially in the last two paragraphs above}

==> Sections/Motivation.tex <==
\section{Motivation}
% AIconfigurator + Astrasim - [network, placement ] not present in AIConfigurator  
% Routing KV cache in P/D disagg case.
% Enhance modeling of AIConfigurator - ^^Not event driven 
% Astrasim - does not support inference , batching 

\subsection{Serving strategy exploration for heterogeneous inference deployments }
% Explain why the serving strategy is a large DSE
Modern inference pipelines must simultaneously accommodate long‑context prompts, multi‑turn interactions, and high request‑level variability, while operating under increasingly strict latency and throughput constraints.
Identifying the optimal LLM serving strategy among a broad set of scheduling parallelism choices, prefill-decode (P/D) and attention–FFN disaggregation (AFD) choices becomes a large design‑space exploration problem, especially for large-scale heterogeneous deployments.
%Evidence through an example
~\Cref{fig:context_length} illustrates the trade‑offs among inference scheduling strategies by exhaustively evaluating nearly 1,300 scheduling configurations, reporting the resulting time‑to‑first‑token (TTFT) across a range of batch sizes (seq/s) for a Qwen3‑30B model deployed on eight H100 GPUs. The number of feasible scheduling choices grows super‑linearly with system scale, particularly in environments with heterogeneous compute nodes and scale‑out interconnects. A key challenge is that exhaustively profiling this expanding design space becomes prohibitively expensive in large‑scale deployments.

% How AIConfigurator++ addresses this limitation
To address this limitation, we employ AIConfigurator++, an event‑driven system modeling framework that captures heterogeneous compute units and accurately estimates data‑transfer latencies using the AstraSim network simulator. This modeling‑ driven approach enables deployment engineers to efficiently identify Pareto‑optimal scheduling strategies as a function of batch size, including the optimal placement of Transformer operators across compute nodes. By modeling system behavior rather than relying on exhaustive profiling, AIConfigurator++ reduces DSE time by $x\%$, making it feasible to explore scheduling policies for large heterogeneous systems spanning diverse compute and interconnect configurations.
Our analysis further reveals that the Pareto‑optimal scheduling configuration is batch‑size dependent. For small batch sizes, prefill–decode (P/D) disaggregation combined with Attention–FFN disaggregation (AFD) yields the minimum TTFT. At medium batch sizes, introducing micro‑batching within AFD improves compute–communication overlap, while at large batch sizes, more aggregated execution schedules are preferred, as they reduce network congestion induced by the large data transfers inherent to AFD. Importantly, the inflection points between these regimes vary with model architecture, cluster topology, and compute‑node heterogeneity, dimensions that we systematically explore in this work.



\begin{comment}
In large‑scale heterogeneous deployments, identifying an optimal LLM serving strategy among a broad set of scheduling policies and attention–FFN disaggregation (AFD) choices becomes a challenging design‑space exploration problem, particularly as the number of transformer blocks increases. This design space spans multiple dimensions.
Along the model‑partitioning dimension, models may be parallelized using tensor parallelism (TP), pipeline parallelism (PP), and expert parallelism (EP). Along the input‑partitioning dimension, requests can be distributed using data parallelism (DP) and sequence parallelism (SP). Importantly, these strategies are composable, enabling compound parallelization schemes for multi‑GPU deployments and significantly expanding the search space.
Figure 6 illustrates the time‑to‑first‑token (TTFT) and ingestion concurrency (requests/s) for a Qwen model on an 8‑GPU system, obtained by brute‑forcing all feasible scheduling configurations. Different colors denote prefill–decode and attention–FFN disaggregation strategies. The results demonstrate that no single configuration is universally optimal; instead, different disaggregation and scheduling choices dominate under different operating regimes. This diversity of optima highlights the need for systematic design‑space exploration to guide efficient LLM serving on future heterogeneous architectures.
\end{comment}

\subsection{Efficient execution of emerging workloads in future system infrastructure}
% Rapidly changing system design with heterogeneous architectures
LLM architectures and system infrastructures are evolving rapidly, a trend expected to further accelerate as AI systems are adopted across an expanding range of application domains. Modern model architectures increasingly extend beyond conventional multi‑head attention (MHA) to incorporate variants such as grouped‑query attention (GQA) and multi‑latent attention (MLA), each exhibiting distinct compute–memory and data‑movement characteristics. In parallel, emerging pipeline techniques such as speculative decoding introduce additional execution heterogeneity, where optimal performance depends on carefully coordinated Attention–FFN disaggregation (AFD) across both draft and verification models. Together, these architectural and pipeline innovations fundamentally reshape the operator scheduling landscape, making optimal placement increasingly sensitive to model structure and execution strategy.

At the same time, system infrastructures are transitioning toward heterogeneous compute platforms. The emergence of architectures such as Rubin CPX~\cite{Rubinmic2}, along with GPU–ASIC combinations including GPU+Groq and GPU+SambaNova designs, reflects a broader shift toward scale‑out clusters composed of specialized accelerators optimized for distinct compute or memory roles. While these heterogeneous platforms significantly expand the design space for inference deployments, they also necessitate fine‑grained operator placement to fully realize their performance potential. Effectively leveraging such systems requires matching LLM operators to compute resources that align with their inherent compute–memory demands.

In this work, we focus on identifying optimal disaggregation strategies for heterogeneous inference deployments. Specifically, we study Attention–FFN disaggregation across diverse Transformer architectures, with case studies centered on context‑length–aware scheduling and the execution of sparse attention and FFN operators. We further evaluate the impact of key architectural parameters—including SRAM capacity, memory bandwidth, and HBM‑backed SRAM designs—across both current and emerging hardware platforms. These detailed analyses illuminate how different workloads benefit from specific system infrastructure choices and provide concrete guidance for future hardware–software co‑design. Overall, by systematically characterizing operator‑level behavior and mapping operators to appropriately matched compute nodes, our approach enables improved resource utilization, reduced latency, and higher overall system efficiency.

\begin{comment}
    

Operator‑ and phase‑level disaggregation introduce significant challenges, as they simultaneously require large volumes of data movement and careful scheduling of operators onto appropriate compute resources. Accurately evaluating these trade‑offs therefore necessitates precise system‑level modeling, particularly for future heterogeneous architectures.
In this paper, we extend NVIDIA AIConfigurator to model attention–FFN disaggregation (AFD). Specifically, we transform the original framework into an event‑driven simulator capable of capturing both the computational costs of AFD and the associated data‑transfer overheads. We further integrate the AstraSim network simulator to accurately estimate interconnect costs and to explore optimal network topologies across different architectural configurations.

AFD partitions the transformer into attention and FFN operators with fundamentally different resource requirements: attention blocks are memory‑bound and demand high memory bandwidth and capacity for KV‑cache storage, while FFN blocks are compute‑intensive and favor devices with high arithmetic throughput. To characterize these differences, we profile each operator across a wide range of GPU platforms spanning multiple generations, with varying HBM capacities and SM counts. Moreover, we evaluate AFD under heterogeneous deployments that combine high‑end GPUs for attention execution with compute‑optimized accelerators featuring large on‑chip SRAMs for FFN execution. By systematically characterizing operator behavior and placing them on appropriately matched compute nodes, our approach enables improved resource utilization, lower latency, and higher overall system efficiency.
\end{comment}

\subsection{Finding the optimal placement of Transformer operators}
Heterogeneous compute modules co‑located within a single cluster—such as GPU–Groq deployments—can be effectively exploited through fine‑grained disaggregation strategies like attention–FFN disaggregation (AFD). In AFD, attention operators are predominantly memory‑bound due to intensive KV‑cache interactions, whereas FFN operators are compute‑bound, making them well‑suited to accelerators with high arithmetic throughput.

However, scheduling fine‑grained operator disaggregation on heterogeneous architectures requires jointly considering compute affinity and data‑movement costs. In particular, effective operator placement must account for compute–communication overlap by co‑locating operators with high data‑exchange requirements on nearby or tightly coupled compute nodes. As shown in Figure XXX, the data‑transfer overhead introduced by fine‑grained disaggregation plays a first‑order role in determining serving throughput.

This work goes beyond modeling heterogeneous architectures by jointly optimizing operator placement and data movement, identifying optimal mappings of attention and FFN operators under fine‑grained AFD to maximize system efficiency.




\begin{comment}
    

Modeling attention–FFN disaggregation (AFD) in large‑scale deployments reveals that merely partitioning attention and FFN operators is insufficient to achieve optimal performance. In addition to disaggregation, the precise placement of these operators onto appropriate compute nodes is critical. As shown in Figure XXX, the cost of data transfer introduced by fine‑grained disaggregation plays a first‑order role in determining serving throughput. Our work goes beyond modeling heterogeneous architectures by jointly optimizing operator placement and data movement, identifying optimal mappings of attention and FFN operators for fine‑grained AFD to maximize system efficiency.
\end{comment}

% Workflow figure - [AIConfigurator++]


\begin{comment}
    Modern large language models (LLMs) exceed the compute and memory capacity of a single accelerator, necessitating distributed execution across multiple devices. Prior work has introduced several orthogonal parallelization strategies to scale LLM training and inference.
Data parallelism (DP) replicates the model across devices and processes different subsets of the input data in parallel. Pipeline parallelism (PP) partitions the model along layer boundaries and assigns successive layers to different devices. Tensor parallelism (TP) shards individual model tensors across devices, enabling a single layer to be computed collaboratively by multiple accelerators. Expert parallelism (EP) distributes experts in Mixture‑of‑Experts (MoE) models across devices, activating only a subset of experts per token. Sequence parallelism (SP) partitions computation along the sequence (token) dimension, distributing tokens from the same input sequence across multiple devices.
Each parallelization strategy exhibits distinct compute–memory trade‑offs and remains sensitive to factors such as model size, hardware topology, and input sequence length. Importantly, these strategies are not mutually exclusive and can be composed to form compound parallelization schemes, giving rise to a large and complex design space for large‑scale deployments.
\end{comment}








==> Sections/Related_Work.tex <==
\section{Related Work}
